An Actionable Framework for Understanding and Improving Talent Retention as a Competitive Advantage in IT Organizations

In the rapidly evolving global business landscape, the demand for software has intensified competition among organizations, leading to challenges in retaining highly qualified IT members in software organizations. One of the problems faced by IT organizations is the retention of these strategic professionals, also known as talent. This work presents an actionable framework for Talent Retention (TR) used in IT organizations. It is based on our findings from interviews performed with 21 IT managers. The TR Framework is our main research outcome. Our framework encompasses a set of factors, contextual characteristics, barriers, strategies, and coping mechanisms. Our findings indicated that software engineers can be differentiated from other professional groups, and beyond competitive salaries, other elements for retaining talent in IT organizations should be considered, such as psychological safety, work-life balance, a positive work environment, innovative and challenging projects, and flexible work. A better understanding of factors could guide IT managers in improving talent management processes by addressing Software Engineering challenges, identifying important elements, and exploring strategies at the individual, team, and organizational levels.

==> tables/old_tab_RQ.tex <==
\begin{table}[h!]
\centering
\caption{Goals addressed in RQ to support the study.}
\label{tab:rq_goals}
\begin{tabular}{p{0.2cm} p{7.3cm}}
\toprule
\textbf{RQ} & \textbf{Goals} 
\\ \midrule
1 & Understanding the factors that influence a talent's decision to stay or leave, as well as obtaining valuable insight into employees' top concerns and motivations.
\\ \midrule
2 & Identifying external factors that may influence organizations' ability to retain talent.
\\ \midrule
3 & Identifying the barriers that IT managers can face when trying to improve the factors that affect the permanence of a talent, such as financial resources, bureaucracy, and skills.
\\ \midrule
4 & Understanding the practices that IT managers are using to retain talent and reduce employee turnover.
\\ \midrule
5 & Gaining insights to identify gaps in talent retention policies beyond existing efforts.
\\ \bottomrule
\end{tabular}

\end{table}
